Projected Walk on Spheres: A Monte Carlo Closest Point Method for Surface PDEs

We present projected walk on spheres (PWoS), a novel pointwise and discretization-free Monte Carlo solver for surface PDEs with Dirichlet boundaries, as a generalization of the walk on spheres method (WoS) [Muller 1956; Sawhney and Crane 2020]. We adapt the recursive relationship of WoS designed for PDEs in volumetric domains to a volumetric neighborhood around the surface, and at the end of each recursion step, we project the sample point on the sphere back to the surface. We motivate this simple modification to WoS with the theory of the closest point extension used in the closest point method. To define the valid volumetric neighborhood domain for PWoS, we develop strategies to estimate the local feature size of the surface and to compute the distance to the Dirichlet boundaries on the surface extended in their normal directions. We also design a mean value filtering method for PWoS to improve the method's efficiency when the surface is represented as a polygonal mesh or a point cloud. Finally, we study the convergence of PWoS and demonstrate its application to graphics tasks, including diffusion curves, geodesic distance computation, and wave propagation animation. We show that our method works with various types of surfaces, including a surface of mixed codimension.

==> Figures/ConvergenceMeanValue/initsamples0.tex <==
1 0.588501
2 0.407464
4 0.291488
8 0.206794
16 0.145287
32 0.105507
64 0.0735271
128 0.0537961
256 0.037914
512 0.0297889
1024 0.0229488


==> Figures/ConvergenceMeanValue/initsamples1.tex <==
1 0.0656843
2 0.0471239
4 0.0428957
8 0.0289666
16 0.0232306
32 0.0215064
64 0.0167396
128 0.0161678
256 0.0160875
512 0.0161164
1024 0.0154125


==> Figures/ConvergenceMeanValue/initsamples10.tex <==
1 0.0140669
2 0.0141751
4 0.0151382
8 0.0145528
16 0.0142628
32 0.0146136
64 0.0142188
128 0.0143552
256 0.0144241
512 0.0144979
1024 0.0145171


==> Figures/ConvergenceMeanValue/mvcsamples0.tex <==
1 0.588501
2 0.588501
4 0.588501
8 0.588501
16 0.588501
32 0.588501
64 0.588501
128 0.588501
256 0.588501
512 0.588501
1024 0.588501


==> Figures/ConvergenceMeanValue/mvcsamples1.tex <==
1 0.44463
2 0.301964
4 0.219794
8 0.162183
16 0.12361
32 0.101198
64 0.0838825
128 0.0744664
256 0.0689533
512 0.0667722
1024 0.0656843


==> Figures/ConvergenceMeanValue/mvcsamples10.tex <==
1 0.318421
2 0.125112
4 0.0869481
8 0.0616553
16 0.0433904
32 0.0294112
64 0.0230296
128 0.0197646
256 0.0166506
512 0.0148364
1024 0.0140669

